Binary Decompilation LLM with Feedback-Driven Multi-Turn Refinement

Binary decompilation is fundamental to security tasks such as vulnerability discovery, malware inspection, and executable-only program understanding. Recent LLM-based decompilation methods have shown promising results, but most still follow a single-turn generation paradigm: given assembly code or decompiler-produced pseudo-code, the model generates one output and stops. Consequently, the generated code may appear readable or even compile successfully, yet still deviate from the behavior of the original binary and mislead downstream analysis. This paper presents AutoDecompiler, a decompilation-specialized LLM trained with reinforcement learning for feedback-driven multi-turn binary decompilation. Instead of treating decompilation as one-shot code generation, AutoDecompiler formulates it as an iterative refinement process, where the model revises generated code based on compilation, execution, and input/output testing feedback. To enable this process, we design decompilation-specific rewards that capture code validity, recompilability, execution consistency, and semantic fidelity. We further construct stage-aware diagnostic feedback from compiler errors, execution failures, and failed test cases, and introduce progress-aware trajectory rewarding and turn-aware advantage reweighting to encourage beneficial revisions while suppressing regressions. We train the AutoDecompiler family and evaluate it across different input settings, model scales, and benchmarks. Experimental results show that AutoDecompiler consistently outperforms its single-turn counterparts under the same model size and input setting, achieving clear improvements in behavioral re-executability. These results demonstrate that learning to exploit program feedback with reinforcement learning is an effective direction for improving the functional correctness of LLM-based binary decompilation.

==> spsections/1introduction1.tex <==
\section{Introduction}
\label{intros}
Binary decompilation aims to recover high-level, C-like source-code representations from low-level executable binaries, enabling analysts to reason about program logic beyond machine instructions\cite{Jakub2017retdec}. % what
It plays a critical role in software security analysis, vulnerability discovery, malware detection, and software maintenance, since most real-world software systems are released only in executable form and their original source code is often unavailable\cite{Wong2025DecLLM,Liu2025TheCS}. % importance
Therefore, practical decompilation requires not only syntactically readable outputs, but also semantic and behavioral consistency with the original binary.


Recent advances in large language models (LLMs) have enabled new possibilities for binary decompilation by leveraging their strong capabilities in code generation and semantic reasoning.
In general, existing LLM-based approaches can be categorized into two paradigms: end-to-end decompilation \cite{Nan2024Nova,feng2024sc2dec,tan2024LLM4Decompile,Liu2025TheCS} and pseudo-code based decompilation \cite{Wong2025DecLLM,hu2024degpt,she2024WaDec,Tan2025SK2DecompileLT,Zhou2025FidelityGPTCD}.
End-to-end methods frame decompilation as a translation task, converting a sequence of assembly instructions into high-level source code in a single-step by leveraging either commercial or fine-tuned LLMs.
Pseudo-code based methods take the pseudo-code representation produced by traditional decompilers as input, leveraging LLMs to analyze and optimize the pseudo-code. 



Despite impressive progress, most existing LLM-based decompilation methods suffer from a fundamental limitation: \textbf{they follow a single-turn generation paradigm, where LLMs reconstruct complete source code from fixed inputs in one pass}. 
In practice, generated code can be compiled, executed, and tested with input/output (I/O) cases, producing diagnostic signals such as compiler errors, runtime exceptions, and failed I/O cases. These signals provide actionable guidance for locating, characterizing, and correcting errors in the generated code, enabling more reliable program recovery. However, current single-turn methods terminate after generation and therefore fail to leverage such feedback for iterative correction and progressive refinement.


These observations highlight the necessity of building decompilation LLMs that can dynamically diagnose, revise, and continuously improve their outputs through compilation and execution feedback.
\textbf{This raises a key research question: how can we transform LLM-based decompilation from a single-turn generation task into a feedback-driven multi-turn refinement process?}


Reinforcement learning (RL) \cite{Wei2025ReinforcingMR,kumar2025iclr-training,jain2025iclrw-multiturn,wang2025deeptrans} provides a natural framework for this problem, as it is designed for sequential decision-making and optimizes policy models through external feedback obtained from interactions with the environment. This makes RL particularly suitable for learning multi-turn refinement behaviors, where each revision depends on prior intermediate outputs and diagnostic signals.



Motivated by this insight, we propose the \textbf{AutoDecompiler}, \textit{a reinforcement-learning-based LLM for feedback-driven multi-turn binary decompilation}. AutoDecompiler iteratively refines an initial decompiled-code candidate by leveraging compilation, execution, and testing feedback to progressively improve semantic and functional correctness.

However, building AutoDecompiler is non-trivial and faces several key challenges:

\noindent\textbf{Challenge 1: Defining reliable rewards for decompilation quality.}
Different from ordinary text generation tasks, the quality of a decompiled program cannot be measured by a single objective.
A desirable decompilation output should be syntactically valid, semantically faithful to the original binary, structurally plausible as C code, and compilable/executable under I/O test cases.
So, how should we design the RL rewards to effectively ensure the decompilation quality?
% Relying only on textual similarity may overlook executable correctness, while relying only on compilation or execution success may encourage code that passes limited checks but deviates from the original binary semantics.


\noindent\textbf{Challenge 2: Converting heterogeneous feedback into effective refinement guidance.}
Compilation and execution feedback provides useful diagnostic signals, but such feedback is often indirect, incomplete, and expressed at different levels of abstraction.
For example, a compiler error may indicate a local syntax or type inconsistency, whereas a failed I/O case only reveals behavioral divergence without directly identifying the faulty statements.

\noindent\textbf{Challenge 3: Preventing harmful refinement across multiple turns.}
Multi-turn refinement does not naturally guarantee monotonic positive improvement.
Although additional refinement turns provide opportunities to repair errors, they also introduce the risk of modifying already-correct code regions, overfitting to local diagnostic feedback, or drifting away from the semantics of the original binary.
In an RL setting, this issue becomes more critical, as the model may learn behaviors that improve immediate rewards while harming long-term semantic fidelity, leading to behavior collapse.

\noindent\textbf{Challenge 4: Assigning proper credit across refinement turns.}
Multi-turn refinement is not a flat generation process: the final output quality is shaped by a sequence of refinement decisions made across different turns.
However, standard policy optimization methods typically assign a shared sequence-level advantage to all generated tokens, ignoring the fact that different refinement turns may contribute unequally to the final improvement.
Such coarse-grained credit assignment makes it difficult for the model to learn which revisions are beneficial, which are ineffective, and which are harmful.



To address the aforementioned challenges, we introduce several novel techniques into AutoDecompiler, each designed to tackle a specific challenge: \textbf{1) Weighted Multi-dimensional Decompilation Reward}. AutoDecompiler designs a multi-dimensional reward that jointly captures syntactic validity, executable correctness, structural plausibility, and semantic fidelity. It first filters invalid outputs using C-like syntax and format constraints, and then evaluates functional correctness by recompiling and executing the candidate against I/O test cases with fine-grained rewards for compilation failures, runtime errors, wrong outputs, and successful executions. Beyond dynamic feedback, AutoDecompiler further incorporates static structural and semantic signals by comparing Abstract Syntax Tree (AST) structures and normalized data-flow dependencies with the source during training. The resulting weighted reward provides a more reliable optimization objective than textual similarity or test-case success alone.
\textbf{2) Structured Diagnostic Feedback Recomposition.} To convert heterogeneous execution-environment signals into actionable refinement guidance, AutoDecompiler introduces a structured diagnostic feedback mechanism. Beyond scalar rewards, it preserves compilation and execution evidence, categorizes failures by stage, and reformulates them into unified natural-language feedback for the next refinement turn. Compilation errors are reported with concrete compiler diagnostics, runtime failures with error messages and execution traces, and I/O mismatches with failing inputs, observed outputs, and expected outputs. This feedback is appended to the conversation history as an environment response, allowing the model to revise code based on explicit diagnostic evidence rather than opaque reward values alone. As a result, AutoDecompiler bridges low-level execution signals and high-level code revision, enabling closed-loop multi-turn decompilation.
\textbf{3) Progress-aware Trajectory Regularization.} 
To prevent harmful refinement across multiple turns, AutoDecompiler augments the final outcome reward with a trajectory-level progress signal. For each refinement trajectory, it first aggregates the multi-dimensional reward at every turn into a scalar score, and then measures the relative improvement between consecutive turns. The overall reward is defined as the final-turn reward plus a weighted average of these progress scores. This design encourages the model to make revisions that consistently increase decompilation quality, while assigning lower reward to trajectories where later edits damage compilation, execution behavior, structural plausibility, or data-flow fidelity. Different from single-turn outcome optimization, this progress-aware regularization supervises the refinement process itself, helping the policy learn when to preserve correct code regions and when to perform targeted repair.
\textbf{4) Turn-aware Advantage Reweighting.}
Multi-turn decompilation refinement requires credit assignment at the level of refinement decisions rather than treating the whole trajectory as a flat generation sequence. AutoDecompiler therefore designs a turn-aware advantage reweighting strategy. For each trajectory, it records the reward vector of every refinement turn, aggregates the reward dimensions into a scalar turn score, and normalizes these scores across valid turns. The resulting turn weights are used to redistribute the trajectory-level advantage back to the token segments generated at different turns. This prevents all revisions from receiving identical supervision and allows the policy to emphasize turns that produce meaningful improvements while suppressing ineffective or damaging edits. By aligning token-level optimization with turn-level refinement quality, AutoDecompiler learns more precise multi-turn repair behaviors.

To make AutoDecompiler applicable to diverse decompilation scenarios and resource constraints, we train a family of AutoDecompiler models under two settings: end-to-end decompilation and pseudo-code-based refinement. These models are further instantiated at three parameter scales, namely 1.3B, 6.7B, and 30B, allowing users to balance decompilation performance and computational cost according to their needs.
Our evaluation spans three benchmarks, HumanEval, MBPP, and ExeBench, and uses three complementary metrics: re-compilability, re-executability\cite{Liu2025TheCS}, and R2I code readability \cite{Eom2024R2I}. The results demonstrate that AutoDecompiler consistently improves over its single-turn counterparts across datasets and model sizes. The gains are particularly pronounced on recompilation and re-execution, showing that feedback-driven multi-turn refinement enables the model to correct concrete syntactic, runtime, and behavioral defects rather than merely producing superficially plausible code. Furthermore, AutoDecompiler remains competitive with similarly sized decompilation models while requiring only about one-tenth of their training data, suggesting that our reward and trajectory-optimization design provides a more sample-efficient path toward reliable LLM-based decompilation.

==> spsections/1introduction2.tex <==
\section{Introduction}
\label{intros}
Binary decompilation aims to recover high-level, C-like source-code representations from low-level executable binaries, enabling analysts to reason about program logic beyond machine instructions\cite{Jakub2017retdec}. % what
It plays a critical role in software security analysis, vulnerability discovery, malware detection, and software maintenance, since most real-world software systems are released only in executable form and their original source code is often unavailable\cite{Wong2025DecLLM,Liu2025TheCS}. % importance
Therefore, practical decompilation requires not only syntactically readable outputs, but also semantic and behavioral consistency with the original binary.


Recent advances in large language models (LLMs) have enabled new possibilities for binary decompilation by leveraging their strong capabilities in code generation and semantic reasoning.
In general, existing LLM-based approaches can be categorized into two paradigms: end-to-end decompilation \cite{Nan2024Nova,feng2024sc2dec,tan2024LLM4Decompile,Liu2025TheCS} and pseudo-code based decompilation \cite{Wong2025DecLLM,hu2024degpt,she2024WaDec,Tan2025SK2DecompileLT,Zhou2025FidelityGPTCD}.
End-to-end methods frame decompilation as a translation task, converting a sequence of assembly instructions into high-level source code in a single-step by leveraging either commercial or fine-tuned LLMs.
Pseudo-code based methods take the pseudo-code representation produced by traditional decompilers as input, leveraging LLMs to analyze and optimize the pseudo-code. 



Despite impressive progress, most existing LLM-based decompilation methods suffer from a fundamental limitation: \textbf{they follow a single-turn generation paradigm, where LLMs reconstruct complete source code from fixed inputs in one pass}. 
In practice, generated code can be compiled, executed, and tested with input/output (I/O) cases, producing diagnostic signals such as compiler errors, runtime exceptions, and failed I/O cases. These signals provide actionable guidance for locating, characterizing, and correcting errors in the generated code, enabling more reliable program recovery. However, current single-turn methods terminate after generation and therefore fail to leverage such feedback for iterative correction and progressive refinement.


These observations highlight the necessity of building decompilation LLMs that can dynamically diagnose, revise, and continuously improve their outputs through compilation and execution feedback.
\textbf{This raises a key research question: how can we transform LLM-based decompilation from a single-turn generation task into a feedback-driven multi-turn refinement process?}


Reinforcement learning (RL) \cite{Wei2025ReinforcingMR,kumar2025iclr-training,jain2025iclrw-multiturn,wang2025deeptrans} provides a natural framework for this problem, as it is designed for sequential decision-making and optimizes policy models through external feedback obtained from interactions with the environment. This makes RL particularly suitable for learning multi-turn refinement behaviors, where each revision depends on prior intermediate outputs and diagnostic signals.



Motivated by this insight, we propose the \textbf{AutoDecompiler}, \textit{a reinforcement-learning-based LLM for feedback-driven multi-turn binary decompilation}. AutoDecompiler iteratively refines an initial decompiled-code candidate by leveraging compilation, execution, and testing feedback to progressively improve semantic and functional correctness.

However, building AutoDecompiler is non-trivial and faces several key challenges:

\noindent\textbf{Challenge 1: Defining reliable rewards for decompilation quality.}
Different from ordinary text generation tasks, the quality of a decompiled program cannot be measured by a single objective.
A desirable decompilation output should be syntactically valid, semantically faithful to the original binary, structurally plausible as C code, and compilable/executable under I/O test cases.
So, how should we design the RL rewards to effectively ensure the decompilation quality?



\noindent\textbf{Challenge 2: Converting heterogeneous feedback into effective refinement guidance.}
Compilation and execution feedback provides useful diagnostic signals, but such feedback is often heterogeneous and weakly localized. Compiler errors, runtime failures, and failed I/O tests reveal different types of abnormal behaviors without directly indicating how to revise the code. Thus, a key challenge is how to transform such feedback into actionable guidance for subsequent refinement turns.


\noindent\textbf{Challenge 3: Ensuring progressive refinement across multiple turns.}
Multi-turn refinement does not naturally guarantee monotonic improvement. Although additional refinement turns provide opportunities to repair previous errors, they may also degrade previously correct behaviors or drift from the original program semantics when responding to local diagnostic feedback. In RL training, this issue is amplified because optimization may favor short-term reward gains while degrading overall decompilation quality.

\noindent\textbf{Challenge 4: Assigning turn-aware credit across refinement turns.}
Multi-turn refinement is not a flat token-generation process: the final decompilation quality is shaped by a sequence of utterance-level refinement decisions made across different turns. However, standard policy optimization methods typically assign a shared sequence advantage to all generated tokens, making the mismatch between token-level optimization and turn-level refinement quality. As a result, beneficial, ineffective, and harmful refinement turns may receive indistinguishable supervision, making it difficult for the model to learn which revisions should be reinforced or suppressed.






To address the aforementioned challenges, we introduce several novel techniques into AutoDecompiler, each designed to tackle the corresponding challenge: \textbf{1) Weighted Multi-dimensional Decompilation Reward}. 
AutoDecompiler designs a multi-dimensional reward that jointly captures C-like validity, executable correctness, syntactic consistency, and semantic fidelity. 
Specifically, a validity-oriented reward penalizes non-C outputs and excessively long hallucinated code; an execution-oriented reward distinguishes compilation failures, runtime errors, incorrect outputs, and successful executions through recompilation and I/O-based testing; and a reference-guided structural-semantic reward further measures AST-level syntactic similarity and data-flow consistency during training. 
These reward components are combined with different weights to provide a more reliable optimization objective for reinforcement learning. \textbf{2) Stage-aware Diagnostic Feedback Construction.} AutoDecompiler introduces a stage-aware diagnostic feedback construction mechanism to bridge low-level execution signals and high-level code refinement. Given a generated code, the environment recompiles and re-executes it against test cases, then returns both a scalar reward and diagnostic feedback. AutoDecompiler further organizes the feedback according to the failure stage, including compilation errors, runtime errors, incorrect outputs, and complete test failures. These stage-specific diagnostics are reformulated into natural-language refinement prompts and fed back to the LLM in the next turn. This design allows the model to exploit concrete failure evidence during iterative decompilation, instead of optimizing from reward values alone. \textbf{3) Progress-aware Trajectory Rewarding.}
To promote progressive refinement across multiple turns, AutoDecompiler augments the final outcome reward with a trajectory-level progress signal. At each turn, the multi-dimensional reward is aggregated into a scalar quality score, and the reward difference between consecutive turns is computed over valid refinement steps. The final trajectory reward combines the final-turn reward with a weighted progress term, thereby favoring trajectories that improve over the initial refinement state and penalizing revisions that reduce compilation correctness, execution behavior, structural similarity, or data-flow consistency. 
\textbf{4) Turn-aware Advantage Reweighting.}
AutoDecompiler introduces a turn-aware advantage reweighting strategy to avoid assigning identical supervision to all generated tokens in a multi-turn trajectory. For each trajectory, it records the reward vector at every refinement turn, aggregates the reward dimensions into a scalar turn score, and normalizes these scores over valid turns to estimate turn-level contributions. The resulting weights redistribute the trajectory-level advantage to the token segments generated at different turns, allowing high-quality refinement turns to receive stronger optimization signals while reducing the reinforcement of low-quality or harmful revisions.




To make AutoDecompiler applicable to diverse decompilation scenarios and resource constraints, we train a family of AutoDecompiler models under two settings: end-to-end decompilation and pseudo-code-based refinement. These models are further instantiated at three parameter scales, namely 1.3B, 6.7B, and 30B, allowing users to balance decompilation performance and computational cost according to their needs.
Our evaluation spans three benchmarks, HumanEval, MBPP, and ExeBench, and uses three complementary metrics: re-compilability, re-executability\cite{Liu2025TheCS}, and R2I code readability \cite{Eom2024R2I}. The results demonstrate that AutoDecompiler consistently improves over its single-turn counterparts across datasets and model sizes. The gains are particularly pronounced on recompilation and re-execution, showing that feedback-driven multi-turn refinement enables the model to correct concrete syntactic, runtime, and behavioral defects rather than merely producing superficially plausible code. Furthermore, AutoDecompiler remains competitive with similarly sized decompilation models while requiring only about one-tenth of their training data, suggesting that our reward and trajectory-optimization design provides a more sample-efficient path toward reliable LLM-based decompilation.
